RewardDance: Reward Scaling in Visual Generation

Reward Models (RMs) are critical for improving generation models via Reinforcement Learning (RL), yet the RM scaling paradigm in visual generation remains largely unexplored. It primarily due to fundamental limitations in existing approaches: CLIP-based RMs suffer from architectural and input modality constraints, while prevalent Bradley-Terry losses are fundamentally misaligned with the next-token prediction mechanism of Vision-Language Models (VLMs), hindering effective scaling. More critically, the RLHF optimization process is plagued by Reward Hacking issue, where models exploit flaws in the reward signal without improving true quality. To address these challenges, we introduce RewardDance, a scalable reward modeling framework that overcomes these barriers through a novel generative reward paradigm. By reformulating the reward score as the model's probability of predicting a "yes" token, indicating that the generated image outperforms a reference image according to specific criteria, RewardDance intrinsically aligns reward objectives with VLM architectures. This alignment unlocks scaling across two dimensions: (1) Model Scaling: Systematic scaling of RMs up to 26 billion parameters; (2) Context Scaling: Integration of task-specific instructions, reference examples, and chain-of-thought (CoT) reasoning. Extensive experiments demonstrate that RewardDance significantly surpasses state-of-the-art methods in text-to-image, text-to-video, and image-to-video generation. Crucially, we resolve the persistent challenge of "reward hacking": Our large-scale RMs exhibit and maintain high reward variance during RL fine-tuning, proving their resistance to hacking and ability to produce diverse, high-quality outputs. It greatly relieves the mode collapse problem that plagues smaller models.

==> sections/abstract.tex <==
\section{abstract}
\begin{abstract}
The rapid advancement of diffusion models has catalyzed remarkable progress in the field of text-to-image generation. However, prevalent models such as Flux, SD3.5 and Midjourney, still grapple with issues like model bias, limited text rendering capabilities, and insufficient understanding of Chinese cultural nuances. To address these limitations, we present Seed T2I, an advanced text-to-image model that excels across diverse dimensions, which adeptly manages Chinese and English prompts, supporting bilingual image generation and text rendering. 
We develop a novel data architecture facilitating knowledge integration and a caption system balancing accuracy and richness. A self-developed bilingual large language model integrated as the text encoder, bestows native Chinese support. Glyph-Aligned ByT5 enables flexible character-level rendering, while Scaled Rope adapts image generation to untrained resolutions. Multi-phase post-training optimizations, including SFT and RLHF iterations, further elevate the model's comprehensive capabilities.
Through extensive experimentation, we demonstrate that Seed T2I achieves state-of-the-art performance across multiple dimensions, including prompt-following, aesthetics, text-rendering, structure accuracy. Furthermore, Seed T2I has been optimized through multiple iterations of RLHF to closely align its outputs with human preferences, as revealed by its outstanding ELO score.
\end{abstract}

